Teaching robots to perceive time -- A reinforcement learning approach (Extended version)

Time perception is the phenomenological experience of time by an individual. In this paper, we study how to replicate neural mechanisms involved in time perception, allowing robots to take a step towards temporal cognition. Our framework follows a twofold biologically inspired approach. The first step consists of estimating the passage of time from sensor measurements, since environmental stimuli influence the perception of time. Sensor data is modeled as Gaussian processes that represent the second-order statistics of the natural environment. The estimated elapsed time between two events is computed from the maximum likelihood estimate of the joint distribution of the data collected between them. Moreover, exactly how time is encoded in the brain remains unknown, but there is strong evidence of the involvement of dopaminergic neurons in timing mechanisms. Since their phasic activity has a similar behavior to the reward prediction error of temporal-difference learning models, the latter are used to replicate this behavior. The second step of this approach consists therefore of applying the agent's estimate of the elapsed time in a reinforcement learning problem, where a feature representation called Microstimuli is used. We validate our framework by applying it to an experiment that was originally conducted with mice, and conclude that a robot using this framework is able to reproduce the timing mechanisms of the animal's brain.

==> From_RL/Abstract_RL.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     File: ExtendedAbstract_abstr.tex                               %
%     Tex Master: ExtendedAbstract.tex                               %
%                                                                    %
%     Author: Andre Calado Marta                                     %
%     Last modified : 2 Dez 2011                                     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The abstract of should have less than 500 words.
% The keywords should be typed here (three to five keywords).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%
%% Abstract
%%
\begin{abstract}
	
Time perception is a concept used to represent the phenomenological experience of time by an individual, present in every activity of our daily lives. Sensory information has been proven to have an impact in the way we perceive the passage of time [citation]. Artificial agents, however, perform their actions based on functions that assume a linear metric of time given by a clock, and lack a variable sense of time that is so prevalent in animals.

The work on this paper focuses on the implementation of a temporal task in a Reinforcement Learning problem, to show how the firing rate of dopaminergic neurons resembles the Temporal-Difference (TD) error in TD learning algorithms. However, TD errors produced by models possessing precise temporal representations, such as those in computers, fail to capture observed patterns of dopaminergic activity. Alternative temporal representations that reflect increasing uncertainty about elapsed time with duration may more accurately capture observed neural and behavioural data from animals, as is the case of Microstimuli. In the implemented problem traditional algorithms are compared to biologically inspired ones, proving the latter not only to correctly represent the dopamine, but also being the most computationally efficient. How time is encoded in the brain remains unknown, but there is strong evidence on the implication of dopamine neurons in timing mechanisms.

This work can be extended by, rather than artificially creating a time basis that is this case is the Microstimuli representation, making the robot obtain this time basis naturally from its navigations through an environment, the same way that happens to humans and animals.

%%
%% Keywords (max 5)
%%

%\begin{IEEEkeywords}
%temporal perception, reinforcement learning, gaussian processes, robotics, microstimuli.
%\end{IEEEkeywords}

%\noindent{{\bf Keywords:}} call centre, call scheduling, weapon and target assignment, dynamic programming, linear programming \\

\end{abstract}



==> From_RL/Conclusion_RL.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     File: ExtendedAbstract_concl.tex                               %
%     Tex Master: ExtendedAbstract.tex                               %
%                                                                    %
%     Author: Andre Calado Marta                                     %
%     Last modified : 27 Dez 2011                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The main conclusions of the study presented in short form.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Conclusions}
\label{section:conclusions}


When it comes to the estimation of time through sensory information, we conclude that, firstly, it is very important to choose a proper way to take care of external information collected by sensors. It was seen that different ways to collect the sensory streams lead to very different results, as well as when it comes to pre-processing techniques such as whitening transformations, being that the whitening transformation to spatially decorrelate the sensory streams provides better results than using them directly as they come, since the statistical properties resemble better those of Gaussian processes with Ornstein-Uhlenbeck covariance functions. 
Furthermore, even though these have before been used to represent the natural statistics of the environment, in this work we compute the numerical likelihood of the sensory streams and conclude that other covariance functions should be tried instead.


In the application of biologically inspired algorithms on reinforcement learning problems, 
The performance of these algorithms implemented as to represent brain functions was compared to that of traditional Q-learning algorithms in a timing task. It can be concluded that
the former are not only more realistic and accurate, but also more efficient that the others. The choice of features plays an important role, being that the Microstimuli representation was shown to be the not only more efficient but also most similar time representation with the dopamine behaviour:
\begin{itemize}
	\item There is uncertainty in the interval boundary between short and long sounds
	\item Uncertainty increases with the length of the interval.
	\item The TD error of TD learning behaves similarly to the dopamine firing rate in the brain, decreasing as a reward starts being expected.
\end{itemize}


==> From_RL/Intro_RL.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     File: ExtendedAbstract_intro.tex                               %
%     Tex Master: ExtendedAbstract.tex                               %
%                                                                    %
%     Author: Andre Calado Marta                                     %
%     Last modified : 27 Dez 2011                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% State the objectives of the work and provide an adequate background,
% avoiding a detailed literature survey or a summary of the results.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Introduction}
\label{sec:intro}

Although a significant amount of information about the human brain has already been discovered, much remains unknown. A possible line of research aims at reproducing specific neural mechanisms using biologically inspired approaches to validate neuro-scientific theories in cyber-physical agents such as robots, as motivated by \cite{IBM} and \cite{STRAND}. One of these mechanisms, commonly referred to as time perception, is a concept used to describe the phenomenological experience of time by an individual \cite{soares2016}, \cite{Gouvea2015}, \cite{Mauk2004}.
Successfully reproducing and implementing this neural mechanism has been attempted using various neural network structures \cite{maniadakis2016}, \cite{Buonomano1995}, \cite{Maniadakis2014}. Giving such temporal cognition to artificial agents might bring new ideas that have not yet been explored and motivates this work. 
In this sense, the reader is invited to consider the (dis)advantages, implications and consequences of having a perception of time, which can be used to explore sentences such as ``Time flies when we are having fun" \cite{soares2016}.

Multiple brain areas, such as the frontal cortex, basal ganglia, parietal cortex, cerebellum, and hippocampus, are known to be responsible for the way we perceive time \cite{Fontes2016}. Not only do different brain parts have different ways of representing time according to the tasks they perform, there is no evidence that only one specific area is responsible for temporal cognition. On the other hand, cyber-physical agents, such as robots, perform tasks based on algorithms that consider time as an external entity, coming from a rigid mechanism (a clock), that ordinarily treats it as an independent variable with its own dimension. 

In this work, we take an initial step towards allowing the time representation of algorithms run by robots to be individually tailored and dynamically applied on its functions. This consists of providing the agent with the tools necessary to estimate the passage of time naturally from, in this case, the information contained within its surroundings. 
Our approach towards this goal is based on extracting temporal information from the environment using sensor data.
However, while the effect of externally collected sensor information on our internal neural mechanisms has been studied \cite{xuan2007}, \cite{Dehaene2003}, \cite{Bruss2010}, the question of how this information should be modelled remains unclear.
Successfully modelling it can contribute to validate the idea that external stimuli influence the perception of time, and prove the hypothesis that time can be estimated from the retrieval of raw information from the agent's sensors. This is in the basis of validating neuroscientifc theories concerning time perception. Furthermore, since neither humans nor animals have an absolute internal clock, it also allows us to study whether such a time estimation can be advantageous for robots when performing certain tasks. For example, if a robot is stopped in a static environment it does not need to know exactly how much time is passing, saving resources. For the area of speech, a consequence of having temporal perception would be enabling robots to learn to adapt their pauses in conversations to the situation and persons involved.


The main question we consider regards how sensor data should be modelled to estimate the perceived passage of time. To the best of the authors' knowledge, the only research in this direction uses a process of stochastic external stimuli to obtain an estimate of time \cite{BI}. This framework forms the basis for this work and is extended by the identification of the parameters of the underlying environmental model, which has not been considered therein.

The main contributions of this paper are the following:

\begin{itemize}
	\item Identifying the hyperparameters of environmental sensor information modelled as Gaussian processes with an Ornstein-Uhlenbeck covariance function. %The sensor information is collected from a cyber-physical agent moving through and environment with a constant movement, such as moving forward or rotating, using cross-validation.
	\item Estimating the perceived elapsed time in a Bayesian inference framework using the identified Gaussian processes and exploring the limitaitons of this approach.
 %Applying a whitening transformation to spatially decorrelate them provides better results than filtering.
%	\item We conclude that the second-order statistics of the natural environment cannot be accurately modeled as Gaussian processes with an Ornstein-Uhlenbeck covariance function.
	\item Application of a Kernel Density Estimation method to analyze the sensor data in a non-parametric way, in order to find suitable models of its statistics.
	% . This approximates the distribution of the data properties and as such can be used to find suitable models of its statistics.

\end{itemize}
One of the ways to represent this phenomena in an artifical agent can be to teach it to estimate the passage of time naturaly, from, for example, the information contained in the surrounding environment. A Reinforcement Learning problem is here conducted using time representations that are supposed to be similar to the ones used within the brain. The contributions are:
\begin{itemize}
	\item Checking how accurate each of these representations is
	\item Even though different time representations have previously been studied, to the best of the authors’ knowledge this has never been applied in a reinforcement learning problem with action selection before.
	\item Compare the efficiency of biologically inspired \textit{vs.} traditional reinforcement learning algorithms.
\end{itemize}

Together with an initial way of estimating time from the environment, the two steps of the problem can give rise to a biologically inspired model in which an agent navigates through an environment, collects information from the sensors and creates an estimate of the time that has elapsed, which can then be converted into a reinforcement learning state that can be used to teach the robot to succeed in a temporal task.

%%%

Section \ref{section:background_RL} focus on the theoretical framework of this work in the neuroscienific field of time perception, and  as in the reinforcement learning concepts this is, a specific function that can be performed using an estimated time, in particular, a reinforcement learning time-dependent task, with the Microstimuli representation, section \ref{section:implementation_RL} focus on its implementation and testing, section \ref{section:results_RL} presents some of the most important results. Finally, in section \ref{section:conclusions_RL}, some conclusions regarding the developed work are taken and future guidelines are defined.


==> From_RL/Step1_RL.tex <==
\section{\textbf{Tabular Markovian Q-learning}}
\label{section:Markov}

With a tabular representation, the action-values are stored in variables and accessed when the value of performing a certain action in a certain state is needed, as well as updated when a reward is received.
In this case, after getting the reward and going to the next state, the agent learns the utility of performing this action in this state by updating the value of that pair state-action:
\begin{equation}
Q(s_t,a_t) \leftarrow Q(s_t,a_t) + \alpha[r_{t+1} + \gamma \max_a Q(s_ {t+1}, a_{t+1}) - Q(s_t,a_t)]
\label{eq:QlearningMain}
\end{equation}
Here, each row of the $Q$-matrix corresponds to a state $s$ and each column to an action $a$, and the crossing between both corresponds $Q(s,a)$, which is the $Q$-value for performing action $a$ in state $s$.

%This process is repeated in each timestep until a final state is reached, independently of having had a positive or negative outcome, representing the end of the trial. In this case, the end of the trial is reached immediately when a certain action is made at a step, for example, when the agent is in the state $s$ of listening to the second sound and in that timestep chooses the incorrect action of pressing a button.

The complete algorithm is represented by pseudo-code in algorithm \ref{alg:Markov}.

\begin{algorithm}
	%\footnotesize
	\caption{Tabular Markovian Q-learning}
	\label{alg:Markov}
	\begin{algorithmic}[1]
		%		\Require
		%		\Statex $M-1$ training sets
		\STATE Initialize $Q$-values table = 0
		\STATE Initialize the Q-learning agent, with $\alpha$ and $\gamma$. 
		\STATE Initialize the explorer, $\epsilon$-greedy
		\STATE Initialize the environment
		\FOR{each episode} 
		\STATE Initialize the agent
		\FOR{each step}
		\STATE $a = \underset{a}{\mathrm{\max}}(Q(s,a))$ %\COMMENT{Perform the action with maximum value for that state}
		\STATE Get the new state $s'$ resulting from performing action $a$ in state $s$, and the corresponding reward, $r$, for that transition.
		\STATE $Q(s,a) = Q(s,a) + \alpha (r+\gamma  \underset{a}{\mathrm{\max}}(Q(s',a))- Q(s,a))$ %\COMMENT{Learning. Update the value for that state and action according to the real reward received}
		\ENDFOR
		\ENDFOR
	\end{algorithmic}
\end{algorithm}

The results are shown in figure \ref{fig:Step1}. It can be seen that the performance of the agent converges to step 3, which means that the agent does all the actions correctly until hearing the second sound, but then does not know which button to press. Again, this is the expected behaviour for a Markovian implementation, and the results can be confirmed in the $Q$-values table \ref{tab:Step1_b}, where values in bold indicate the less negative action to do in each state, therefore the one that the agent will prefer to choose. In the state ``Init", the action with the highest value is the ``Start", in the ``Interval" between two sounds, the agent correctly does the action ``Wait", but then when it is in the ``Sound" state, it does not have enough information to decide if is hearing the first or second sound, therefore always does the action corresponding to the first one, that is ``Wait".
\begin{figure}[!htp]
	\centering
	\includegraphics[width=0.4\textwidth]{Figures/Step1_results.png}
	\caption[Tabular Markovian algorithm]{Tabular Markovian algorithm. The $x$-axis of the figures represent each of the 1000 episodes, and the $y$-axis the final step reached during each of the episodes, which is equivalent to the performance of the agent during that episode.}
	\label{fig:Step1}
\end{figure}


\begin{table}[]
	\centering
	\caption[$Q$-values for tabular Markovian Q-learning]{$Q$-values for tabular Markovian Q-learning.}
	\label{tab:Step1_a}
	\begin{tabular}{cc|cccc}
		\hline
		\multicolumn{2}{c|}{\multirow{2}{*}{Q(s, a)}} & \multicolumn{4}{c}{Actions}            \\
		\multicolumn{2}{c|}{}                         & Start      & Wait      & Short & Long  \\ \hline
		\multirow{3}{*}{\rotatebox[origin=c]{90}{States}}       & Init          & \textbf{2.1716e-05} & \textbf{1.947e-05} & -0.99 & -0.99 \\
		& Sound         & -0.99      & \textbf{5.210e-56} & -0.85 & -0.49 \\
		& Interval      & -0.99      & \textbf{5.452e-57} & -0.99 & -0.99
	\end{tabular}
\end{table}



==> From_RL/Step2_RL.tex <==

\section{\textbf{Tabular non-Markovian Q-learning}}
\label{section:nonMarkov}

Unlike previously, in this case a list of the previous states is given to the agent with their history. This transforms the problem in a trivial one, but in order to properly estimate the duration, more information needed to be provided to the agent than just the current state. It needs to know at least the number of states between the first and second tones to be able to make a proper decision. 

\begin{figure}[!h]
	\footnotesize
	\centering
	\includegraphics[width=0.4\textwidth]{Figures/Step2_results.png}
	\caption[Tabular non-Markovian Q-learning]{Performance of the tabular non-Markovian Q-learning algorithm, over 1400 episodes.}
	\label{fig:Step2}
\end{figure}

\begin{table}[]
	\centering
	\caption{Computational resources required by the tabular non-Markovian Q-learning approach.}
	\label{tab:Step2}
	\begin{tabular}{lllll}
		\hline
		Interval & Processing Time & Dict. size & Table size & Converges in  \\ \hline
		2    & 1.37 & 30 & 120 & 20 \\
		4    & 2.07 & 363 & 1452 & 60 \\
		6	 & 1.96 & 3,279	 & 13116 & 63 \\ 
		8    & 2.40 & 29,523  & 118,128 & 115 \\
		10    & 6.35 & 265,719 & 1,062,876 & 90 \\
		12    & 35.28 & 2,391,483 & 9,565,932 & 160 \\
		14    & 395.06 & 21,523,359	& 86,093,436 & 135 \\ \hline
	\end{tabular}
\end{table}


\begin{table}[]
	\centering
	\caption[$Q$-values for tabular non-Markovian Q-learning]{$Q$-values for tabular non-Markovian Q-learning}
	\label{tab:Step1_b}
	\begin{tabular}{cc|cccc}
		\hline
		\multicolumn{2}{c|}{\multirow{2}{*}{Q(s, a)}} & \multicolumn{4}{c}{Actions}   \\
		\multicolumn{2}{c|}{}                         & Start & Wait  & Short & Long  \\ \hline
		\multirow{3}{*}{\rotatebox[origin=c]{90}{States}}       & Init          & \textbf{-0.28} & -1.13 & -1.14 & -1.14 \\
		& Sound         & -1.15 &\textbf{ -0.59} & -1.16 & -1.13 \\
		& Interval      & -1.12 & \textbf{-0.07} & -1.11 & -1.10
	\end{tabular}
\end{table}
As seen in figure \ref{fig:Step2}, around episode 80 the agent already knows the correct sequence of actions to perform as to maximize the amount of reward.

Even though it solves the timing problem, this algorithm comes with the disadvantage of demanding a big amount of computational resources such as memory and processing time, which will increase exponentially with the increase of the maximum interval between the two sounds. The values for the usage of these resources are represented in table \ref{tab:Step2}. The first column is the maximum interval between the two sounds, in timesteps, the second is the processing time it takes for the algorithm to do 1400 iterations, the two next are the number of rows of the dictionary and table, respectively, and the last column is the episode in which the agent learns the sequence of actions to perform.


==> From_RL/Step3_RL.tex <==

\section{\textbf{Function Approximation with CSC representation}}
\label{section:FA_CSC}

In the case of function approximation, each singular state is not directly saved in memory, rather, is represented as a set of features:
\begin{equation}
Q(s,a) = \sum_{i=1}^d w_i \phi_i (s,a),
\label{eq:Qfeatures}
\end{equation} This is something that seems natural to better represent the brain mechanisms, and can be applied for larger problems as well as speed up learning. 
However, a proper choice of features is absolutely necessary for the success of the algorithm. 
\begin{equation}
\begin{aligned}
w_{t+1}(d) &= w_t(d) + \alpha \delta_t e_t(d) \\
\delta_t &= r_t + \gamma Q(s_{t+1}) - Q(s_t) \\
e_{t+1}(d) &= \gamma \lambda e_t(d) + x_t(d) \\
\end{aligned}
\label{eq:Qweights}
\end{equation}

\begin{algorithm}
	\footnotesize
	\caption{Q-learning with Function Approximation}
	\label{alg:FA}
	\begin{algorithmic}[1]
		%		\Require
		\STATE Initialize $Q(s,a) = 0$
		\STATE Initialize $w=[w_{1},w_{2},...,w_{n}]$ randomly (e.g. $w_{i} \in [0,1]$)
		\FOR{each repetition} 
		\FOR{each episode}
		\STATE Initialize $s$
		\FOR{each step}
		\STATE Choose $a$ from $s$ using policy derived from Q (e.g: $\epsilon$-greedy) %\COMMENT{$\epsilon-greedy$}
		\STATE Take action $a$, observe $r$, $s’$
		\STATE $\delta = [r + \gamma \max a' Q(s’,a’)] – Q(s,a)$
		\STATE $e_{traces n} \gets \gamma \lambda e_{traces n} + x_{n}$
		\STATE $w_{n}(a) \gets w_{n}(a) + \alpha \delta e_{traces n}$
		\STATE $s \gets s'$
		\ENDFOR
		\STATE Until $s$ is terminal
		\ENDFOR
		\ENDFOR
	\end{algorithmic}
\end{algorithm}

In this case, the choice of features $x_{n}$ in line 9 of algorithm \ref{alg:FA} is considered to be given by a Complete Serial Compound (CSC) time representation, described in \eqref{eq:CSC}.
\begin{equation}
x_{i,j}(t)=\begin{cases}
1 , & \text{if element $j$ of stimuli $i$ is present in } t.\\
0, & \text{otherwise.}
\end{cases}
\label{eq:CSC}
\end{equation}

\begin{table}[]
	\centering
	\caption[Properties of CSC with function approximation]{Properties of the function approximation approach with the CSC time representation. The first and last columns are in timesteps, and the second one is the computational time it takes to compute.}
	\label{tab:Step3}
	\begin{tabular}{lllll}
		\hline
		\begin{tabular}[c]{@{}l@{}}Maximum\\   Interval\end{tabular} & Time (s) & Features' size& Weights' size& Converges in \\ \hline
		2 & 19.6 & 6 & 24 & 200 \\
		4 & 24.2 & 8 &32 & 150 \\
		8 & 41.5 & 12 & 48 & 260 \\
		10 & 54.0 & 14 & 56 & 400 \\
		12 & 66.5 & 16& 64 & 410 \\
		16 & 70.9 & 20& 80 & 500 \\
		20 & 104.9 & 24& 96 & 600 \\
		30 & 176.9 & 34& 136 & 800
	\end{tabular}
\end{table}

\begin{figure}[!h]
	\centering
	\includegraphics[width=0.4\textwidth]{Figures/Step3_results.png}
	\caption[Convergence graph of Step 3]{Convergence graph of Q-learning with CSC representation for a temporal discrimination task.}
	\label{fig:Step3}
\end{figure}

The problem is limited by the number of features that can be used, which can be biologically seen as memory constraints, making it impossible to save all past events. Here there is no generalization between time instants, since only one feature is active for each stimulus.


==> From_RL/Step4_RL.tex <==

\section{\textbf{Function Approximation with Microstimuli representation}}
\label{section:FA_MS}

On the other hand, with the Microstimuli representation a set of features is triggered every time there is a stimulus or a reward. 
The same Q-learning with function approximation algorithm \ref{alg:FA} is used, but now the features are encoded according to figure \ref{fig:MScreation}, in which a set of temporal basis functions, represented in the middle by Gaussians, are uniformly distributed along the trace height, in the left. The features are then a function of the basis functions represented by
\begin{figure}[!htp]
	\centering
	\includegraphics[width=0.5\textwidth]{Figures/MicrostimuliCreation.png}
	\caption[Microstimuli creation]{Microstimuli creation. Extracted from \cite{Elliot2008}}
	\label{fig:MScreation}
\end{figure}
\begin{equation}
x_{t}(i) = y_{t} \times f(y_{t}, \frac{i}{m}, \sigma),
\label{eq:MS1}
\end{equation}
where $m$ is the number of microstimuli per stimulus, $i$ is the total number of microstimuli, $x_{t}(i)$ is the level of each existing microstimuli at time $t$, and $y_{t}$ the trace height. $f(y, \mu, \sigma)$ are the basis functions, that, if Gaussians, are given by
\begin{equation} 
f(y, \mu, \sigma) = \frac{1}{\sqrt{2 \pi}} \exp( - \frac{(y - \mu)^2}{2 \sigma^2}).
\label{eq:MS2}
\end{equation}
As Gaussians, $\mu$ is the centre and $\sigma$ the width of each basis function. $y_{t}$ decays exponentially according to 
\begin{equation} 
y_{t} = \exp(- (1-decay) \times t).
\label{eq:MS3}
\end{equation}

\begin{figure}[!htp]
	\centering
	\includegraphics[width=0.4\textwidth]{Figures/MS_8.png}
	\caption{Convergence graph of Q-learning with Microstimuli for a temporal discrimination task. Maximum interval $=$ 8 timesteps.}
	\label{fig:MS_8}
\end{figure}
\begin{figure}[!htp]
	\centering
	\includegraphics[width=0.3\textwidth]{Figures/MS_8b.png}
	\caption{Number of intervals wrongly classified according to their corresponding duration. The maximum interval duration was 8 timesteps.}
	\label{fig:MS_8a}
\end{figure}

The previously described behaviour of the algorithm can be seen in figure \ref{fig:MS_8}, where the algorithm does not converge due to the incorrectly classified intervals in the boundary, as shown in figure \ref{fig:MS_8a}. Here it can be compared with the one of the mice performing the experiment in the paper \cite{soares2016}, showing that the agent behaves similarly to the way as mice did in the original experiment.

In table \ref{tab:MSdata} are shown the computational characteristics of this algorithm, implemented for 7000 trials, while the other algorithms were for 1000.
\begin{table}[]
	\centering
	\caption{Microstimuli characteristics}
	\label{tab:MSdata}
	\begin{tabular}{cccc}
		\hline
		\begin{tabular}[c]{@{}c@{}}Maximum\\ interval\end{tabular} & Time (s) & \begin{tabular}[c]{@{}c@{}}Size of features \\ and weights\end{tabular} & \begin{tabular}[c]{@{}c@{}}Converges in\\ (last outside \\ border)\end{tabular} \\ \hline
		2 & 34.3 & 31, 124 & 1000 \\
		4 & 47.4 & 31, 124 & 750 \\
		6 & 54.02 & 31, 124 & 627 \\
		8 & 54.1 & 31, 124 & 969 \\
		10 & 56.4 & 31, 124 & 1300 \\
		12 & 66.8 & 31, 124 & 2500 (1100) \\
		14 & 78.8 & 31, 124 & 1295 ( 789) \\
		16 & 91.1 & 31, 124 & 1124 ( 984) \\
		18 & 82.5 & 31, 124 & 1745 (969) \\
		20 & 90.7 & 31, 124 & 2274(2274) \\
		22 & 99.2 & 31, 124 & 1621 (1388) \\
		30 & 126.2 & 31, 124 & 6800 (3400)
	\end{tabular}
\end{table}

The comparison with the previous algorithms is shown in figure \ref{fig:Comparison}, and is the collection of values from tables \ref{tab:Step2} and \ref{tab:MSdata}.
\begin{figure}[!h]
	\centering
	\includegraphics[width=0.5\textwidth]{Figures/Comparison.png}
	\caption[Comparison of the algorithms]{Comparison of the computational time of the tested algorithms.}
	\label{fig:Comparison}
\end{figure}
The problem of the previous algorithms is that, if we want to increase the duration of the interval to be timed or, even keeping this fixed, increasing the temporal discretization, then the computational requirements become too demanding. On the other hand, with Microstimuli representation even if the interval increases the number of features remains the same, being more scalable.



==> From_RL/background_RL.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     File: ExtendedAbstract_imple.tex                               %
%     Tex Master: ExtendedAbstract.tex                               %
%                                                                    %
%     Author: Andre Calado Marta                                     %
%     Last modified : 27 Dez 2011                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% A Calculation section represents a practical development
% from a theoretical basis.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Background}
\label{section:background_RL}


\subsection{Neurosciences}
\label{ssection:framwork_ms}

%Papers such as \cite{Niv2011} and \cite{York2009} provide an excellent baseline for the reinforcement learning fundamentals and how these should be considered such that brain functions, particularly those ruled by dopamine neurotransmitters, are reproduced as correctly as possible. In specific, when it comes to the behaviour of the Reward Prediction Error (RPE) already mentioned in chapter \ref{section:background}. 


This paper focuses on the second part of the whole problem suggested, that assumes that an artificial agent has some source of temporal information, and has to use that information to perform its tasks. This source can be a clock, as is the case in most of the current algorithms, or can be something biologically inspired, such as the framework explained in the previous chapter, in which the temporal source is a sensory-based clock.
One of the ways in which it is possible to test the role of time representation is in reinforcement learning problems that aim at solving time-dependent tasks.

A relevant question at this point is how time is represented in a reinforcement learning task, in a way that correctly represents what is already known about the timing mechanisms in the brain. This is the main focus of this chapter, alongside with a comparison between these and traditional algorithms that do not consider a specific time representation, in order to test how well these can perform in timing tasks. 

From \cite{maia2009} it can be said that in RL models of the Basal Ganglia, cortical inputs to the Striatum are what makes this structure encode the estimated value of time, being these inputs the basis of the feature representation. The set of features $\phi(s,a)$ in equation \eqref{eq:Qfeatures} is what represents a RL state and is believed to be where some of the aspects of an animal's experience are encoded. In this scenario, the strengths of the corticostriatal synapses are the ones represented by the set of weights ${w_{t}(1), …, w_{t}(d)}$ from the same equation. These weights can be updated in fucntion-approximation reinforcement learning problems.

Based on this, the two main theories used nowadays to represent stimulus, given the need of consistency with what happens in the Basal Ganglia, are:

\textbf{Presence}, ...

\textbf{Complete Serial Compound}, or CSC, \cite{montague1996} \cite{sutton1990}, is the current standard representation in TD models. It considers each feature as a timestep of the stimulus, since its onset. This means that, in order to know how many timesteps have passed since the stimulus happened, the only thing needed is counting the number of features that was activated, which corresponds to a perfect clock notion. Even though this representation is useful for the examination of TD learning rules, it presents inconsistencies in representing characteristics of the dopamine system \cite{daw2006}.

\textbf{Microstimuli} came up as an alternative time representation in \cite{Elliot2008}. A number of microstimuli are deploited by a stimulus, and, as time goes by, different sets of microstimuli become more or less active since later ones are wider, shorter and have a later peak. So knowing how much a microstimulus has decayed due to its slowly decaying memory trace can be seen as a basis for the elapsed time, providing a coarse code of the trace height.

%The latter is the most consistent with what happens in the basal ganglia, where neurons encode timestamps of different events but more recent time points are more precisely decoded than later ones. This is present in the Microstimuli characteristic of later microstimuli being more dispersed than recent ones, having a smaller temporal precision but taking the credit for the reward spread over a bigger number of microstimuli.
%It considers that both cues and rewards elicit their own set of microstimuli, which encode a kind of uncertainty in the temporal prediction. It has indeed been found by \cite{Fiorillo2008} that, as the interval duration to be estimated increases, the dopamine response to the reward also increases, whereas to the cue it decreases, supporting this theory.

\subsection{Reinforcement learning}
\label{ssection:framwork_rl}

An example of a time-dependent task in which the time estimate can be used is teaching an artificial agent how to act in an environment in order to reach a certain goal, using a Temporal-Difference learning algorithm is presented in section \ref{subsection:reinflearning}, and described by \eqref{eq:QlearningMain}. The goal is to specifically estimate the sequence of actions to perform in a certain task. For this, four variations of Q-learning are implemented for the same task, with the goal of being compared, and, particularly, understanding whether variations that include a realistic time representation, such as Microstimuli, may prove to be more useful and efficient than others that have been the baseline until now and rely on a perfect clock instead. 

A task similar to the one explained in \cite{soares2016} with mice was implemented in an experiment with an artificial agent, in order to compare the results with the ones verified in the original one. In this experiment, the agent is, at each timestep, in any of three states: $S = {\text{0) Init, 1) Sound, 2) Wait}}$, and in each of them can choose any of four actions: $A = {\text{Start, Wait, Short, Long}}$. The setup of the experiment consists on three buttons that the agent can choose to press: A ``Start" button, that, if pressed in the beginning of the experiment, initializes it and gives rise to the appearance of two equal sounds separated by a certain time interval, i.e, a certain number of timesteps between them. The choice of the interval duration is done based on 50\% of probability of being short, and 50\% of being long. Inside the chosen interval, there is an uniform probability of choosing any value within that interval. The action ``Wait" corresponds to the agent doing an action that does not interfere with the state of the experiment, which means that no button is pressed at that timestep. If the agent correctly presses the ``Start" button to start the experiment and does the action ``Wait” until hearing the first and second sounds, then it has to, according to the perceived duration of the interval between the two, press the ``Short" or ``Long" button. If the button corresponding to the correct interval duration is pressed, then a reward signal is given to the agent. Otherwise, it gets a negative reward corresponding to a punishment. In the real experiment this corresponds to giving either water/food or an unpleasant sound, respectively. The schematic representation of the experiment can be seen if figure \ref{fig:RLtask}.

%\begin{table}[]
%	\centering
%	\caption[Reinforcement learning time-dependent task]{Setup of the RL time-dependent task. The value of the intersection between a row, $s_{t}$, and a column, $a_{t}$, indicates the state $s_{t+1}$ for which the agent goes in the next timestep. N means that the agent gets a negative reward, and Y a positive, and in both cases the experiment end. In all the others the reward is neutral, $r_{t}=0$.}
%	\label{tab:RLtask}
%	\begin{tabular}{lllllll}
%		\cline{4-7}
%		\multicolumn{3}{l}{\multirow{2}{*}{}} & \multicolumn{4}{l}{Actions} \\
%		\multicolumn{3}{l}{} & Start & Wait & Short & Long \\ \cline{4-7} 
%		\multirow{3}{*}{\rotatebox[origin=c]{90}{States}} & 0) & \multicolumn{1}{l|}{Init} & 1 & 0 & N & N \\
%		& 1) & \multicolumn{1}{l|}{Sound} & N & 1 or 2 & N or Y & N or Y \\
%		& 2) & \multicolumn{1}{l|}{Interval} & N & 1 or 2 & N & N
%	\end{tabular}
%\end{table}

\begin{figure}[!h]
	\centering
	\includegraphics[width=0.5\textwidth]{Figures/RLexpMice.png}
	\caption[RL task]{RL task. The horizontal line represents the passage of time, from left to right, in which the timesteps are constant and from one to the next there is always a state transition. The sequence of states shown is the optimal one in case the agent chooses the corresponding actions in blue. The last action to choose can be either Short or Long according to the number of states "Interval" that exist, and the reward is given after that last action is taken.}
	\label{fig:RLtask}
\end{figure}

In each episode, the algorithm's performance is evaluated in 5 steps, that show how well the agent behaved in that episode:
%\newcounter{enumi2}
\begin{enumerate}
	\footnotesize
	\setcounter{enumi}{-1}
	\item Did not press the ``Start" button.
	\item Presses the button ``Start”.
	\item Waits after hearing the first sound.
	\item Waits as many times as needed, until hearing the second sound.
	\item Makes the correct choice according to the length of the interval.
\end{enumerate}

The four variations of Q-learning implemented for this same task with the goal of being compared are described ahead.



==> L4DC_Problem_formulation.tex <==

\section{Problem Formulation}
\label{section:L4DC_Problem_formulation}


The question of giving a robot the ability to measure the passage of time posed in this work is divided in the two main problems presented next.
%Explain clearly how we are going to do both:


\begin{problem}[From Sensing to Time]
Understand whether we can give a robot the sense of the passage of time - Given observations $\mathcal{O}$, compute the MAP estimate of \eqref{eq:bayesian} to find the $\tau$ that corresponds to the perceived elapsed time.
\label{problem1}
\end{problem}
We assume that $N$ observations are taken uniformly throughout the elapsed time $\tau$ at time instances $t_1, \dots, t_N$, from $i = 1,\dots,M$ independent sensors. The observations are denoted as $\mathcal{O} = \{y_i\}_{i=1}^{M}$, where $y_i$ is a $N$-dimensional vector given by $[y_{i}(t_{1}), \dots,y_{i}(t_{N})]^T$. 
The probability of having observed $\mathcal{O}$ during the interval $\tau$ is modelled as a zero-mean joint Gaussian distribution over the observations of all sensors, with covariance $K$:
\begin{equation}
p(y_{i}|\tau) = \mathcal{N}(y_i; 0, K(\theta)) = \dfrac{1}{\sqrt{\det(2\pi K(\theta))}} e^{-\frac{1}{2}y_{i}K(\theta)^{-1}y_{i}^T}.
\label{eq:equationBI} 
\end{equation}
This expression corresponds to the likelihood $p(\mathcal{O}|\tau)$ in \eqref{eq:bayesian}, and therefore the solution to Problem \ref{problem1} is the  maximum of the joint distribution, which is the maximum likelihood estimate and corresponds in this case to the MAP estimate of the elapsed time $\tau$.

To solve Problem \ref{problem1} we need to extend the work done in \cite{BI} by estimating the hyperparameters of the model from data. \\

\textbf{Problem 1.1 (Hyperparameter identification)}
\textit{Use Bayesian model selection to find the model's hyperparameters, $\theta$.}\\

To find $\theta$, we maximize the logarithm of the marginal likelihood in \eqref{eq:equationBI} with respect to the parameters $\theta$ of $K$, which involves computing the respective derivatives:
\begin{equation}
\frac{\partial}{\partial\theta_j} \log p(y|\theta) = -\frac{1}{2} tr((\alpha\alpha^T - K^{-1} ) \frac{\partial K}{\partial\theta_j}, \text{ where } \alpha = K^{-1} y
\label{eq:Gderivates}
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{problem}[From Time to Action] 
Study whether a robot can correctly use its estimate of the elapsed time to perform a time-dependent task.
\label{problem2}
\end{problem}
To test how accurate the estimate is, we use it in a reinforcement learning problem with action selection. Since we are interested in the value of each action, we use Q-learning with linear function approximation, so \eqref{eq:V-value} thus becomes: 
\begin{equation}
Q(s,a) = \sum_{i=1}^d w_i x_i (s,a),
\label{eq:Qfeatures}
\end{equation}\\
where each feature $x$ is represented by a set of microstimuli given by \eqref{eq:MS1}. The weights $w_i$ represent the values that indicate how important each feature is for each particular state and action, and, together with $\delta$ and $e$, are updated according to:
\begin{equation}
\begin{aligned}
w_{t+1}(d) &= w_t(d) + \alpha \delta_t e_t(d) \\
\delta_t &= r_t + \gamma Q(s_{t+1}) - Q(s_t) \\
e_{t+1}(d) &= \gamma \Lambda e_t(d) + x_t(d).
\end{aligned}
\label{eq:Qweights}
\end{equation}
The TD error, denoted by $\delta$, is the difference between the reward $r$ received and the expected one, at each timestep. The eligibility traces are denoted by $e$, and, multiplied by the TD error, expand the influence of the presence of a state through time, influencing the weight $w$ given to each one on the responsibility of a certain reward received. The decay parameter that determines the plasticity window of recent stimuli is $\Lambda$.

Problem \ref{problem2} is solved by analysing the results of this TD learning framework using \textit{microstimuli}. If they successfully replicate a real experiment where time perception is needed, we claim that we were able to give some temporal cognition to the agent.


==> L4DC_RL.tex <==
\section{Replicating the perception of time using reinforcement learning}
\label{section:L4DC_RL}

% Total formulation and how we solve it.

%A robot has been trained to collect data $\mathcal{O}$ from its sensors while walking around a room, and with that data estimate time. Now it is running online. 
In this section, the frameworks used to approach both problems posed in Sections \ref{ssection:bayesian_framework} and \ref{ssection:problem_time_to_action} are merged. By combining them, we obtain our third and most important problem in this paper: \textit{Can a robot correctly use its estimate of the elapsed time to perform a time-dependent task?}

To explore this, consider a reinforcement learning setup in which a robot is navigating around an environment. It receives a stimulus indicating that it should start measuring time and starts recording the data received in its sensors. Later, a second stimulus tells the robot to stop measuring data and estimate how much time has passed since the first stimulus, based on the data it collected (Section \ref{ssection:bayesian_framework}). Intuitively, this consists on measuring how much the data points have changed.  

%\begin{assumption}[Model selection]
\textbf{Assumption 1 (Model selection)}
\textit{Assume that the data follows a Gaussian process with Ornstein-Uhlenbeck covariance \eqref{eq:OU}. }\\
%\end{assumption}
In this case, the $N \times N$ Ornstein-Uhlenbeck covariance matrix $K(\tau)$, where $\tau = i-j$, is given by: 
\begin{equation}
K(\tau) = e^{-\lambda |\tau|} + \sigma^2 \delta(\tau) \text{, where } \delta(\tau) = \begin{cases}
    1,& \text{if } \tau =0\\
    0,              & \text{otherwise}
\end{cases},
\label{eq:OU}
\end{equation}
where $\lambda$ and $\sigma$ are the parameters $\theta$ of the covariance $K$, called hyperparameters of the model in the context of the Bayesian framework. By finding the appropriate values for $\lambda$ and $\sigma$, the properties of the Gaussian process should approximate the ones of the data. 
%In \eqref{eq:Gderivates}, $\theta$ is thus the vector of parameters $[\lambda, \sigma]$ so
%\begin{equation} 
%\begin{aligned}
%\frac{\partial K_{i}(\tau)}{\partial \lambda} =-|\tau| \exp (-\lambda|\tau|) \text{   and   } \frac{\partial K_{i}(\tau)}{\partial \sigma} =2 \sigma \delta(\tau).
%\end{aligned}
%\end{equation}
We thus obtain a value for $\tau$ that corresponds to the estimate of the robot of the elapsed time between the two stimuli.

Afterwards, this estimate is used by the features of the reinforcement learning problem: a set of microstimuli is deployed in both the features of the initial state, where the robot perceived the first stimulus, and in the ones of the state corresponding to the estimated $\tau$. In summary, this estimate of the elapsed time $\tau$ influences the timestep of the algorithm at which a new set of microstimuli is deployed in the features $x$, which influences the value $Q$ of the pair state-action and therefore the action $a$ chosen by the agent.

By comparing the actions of a robot with those of a real agent, such as a mouse, in the same experiment, we can thus find out wheter the robot obtained a sense of the passage of time similar to the one of a real agent or not. That is, we are able to answer the thrid question of this work -- whether the robot able to estimate correctly the passage of time and use it to perform a time-dependent task. 
Using the TD algorihm the robot should therefore learn to do an action corresponding to naviageting aronud the environment after seeing the first stimulus, and an action corresponding to the estimated interval between the two stimuli after seeing the second (Section \ref{ssection:problem_time_to_action}). as expected, the choice of which action to choose depends on how well it estimated the elapsed time, being the Q-values learned over multiple episodes. This framework is presented in algorithm \ref{alg:RL}.

\begin{algorithm}[h]
	%\footnotesize
	\caption{From sensing to action based on perceived time}
	\label{alg:RL}
	\begin{algorithmic}[1]
		%		\Require
		\STATE Initialize $Q(s,a) = 0$, for all $s \in \mathcal{S}$, $a \in \mathcal{A}$
		\STATE Initialize $w_{1},\dots,w_d$ randomly (e.g. $w_{i} \in [0,1]$)
		\FOR{each episode}
		\FOR{each timestep $t$}
			\STATE Initialize $s$
			\IF{first stimulus == 1}
				\STATE Update $x_t(1), \dots ,x_t(d)$ according to \eqref{eq:MS1}
				%\STATE (action should be random walk)
			\ELSIF{has received stimulus 1 but not 2}
				\STATE collect data $y_t(1), \dots ,y_t(M)$
				%\STATE (action should be press button short/long)
			\ELSIF{second stimulus == 2}
				\STATE Compute the estimate of the elapsed time, $\tau$, from \eqref{eq:equationBI}
				\STATE Update $x_\tau(1), \dots ,x_\tau(d)$ according to \eqref{eq:MS1}
				%\STATE (action should be press button short/long)		
			\ENDIF
			\STATE Choose $a_t$ from $s_t$ using policy derived from Q
			\STATE Take action $a_t$, observe $r_t$, $s_{t+1}$
			\STATE $\delta = [r_t + \gamma \max_{a_{t+1}} Q(s_{t+1},a_{t+1})] – Q(s_t,a_t)$
			\STATE $e_{traces n} \gets \gamma \Lambda e_{traces n} + x_{n}$
			\STATE $w_{n}(a) \gets w_{n}(a) + \alpha \delta e_{traces n}$
			\STATE $s_t \gets s_{t+1}$
		\ENDFOR
		\STATE Until $s$ is terminal
		\ENDFOR
	\end{algorithmic}
\end{algorithm}

%\begin{algorithm}
%	\caption{From sensing to action based on perceived time}
%	\label{alg:RL}
%	\begin{algorithmic}[1]
%		%		\Require
%		\STATE Initialize $Q(s,a) = 0$
%		\STATE Initialize $w=[w_{1},w_{2},...,w_{n}]$ randomly (e.g. $w_{i} \in [0,1]$)
%		\FOR{each episode}
%			\STATE Initialize $s$
%			\WHILE{there isnt any tone}
%				\STATE Do action = random walk
%			\ENDWHILE
%			% first tone == 1
%			\STATE features = MS
%			\WHILE{it doesnt hear the second tone}
%				\STATE save data obtained from sensors
%				\STATE Do action = random walk
%			\ENDWHILE
%			% second tone == 2
%			\STATE Compute the estimate of the elapsed time, $\tau$, from eq.1
%			\STATE features = MS in tau.				
%
%			\STATE Choose $a$ from $s$ using policy derived from Q
%			\STATE Take action $a$, observe $r$, $s’$
%			\STATE $\delta = [r + \gamma \max a' Q(s’,a’)] – Q(s,a)$
%			\STATE $e_{traces n} \gets \gamma \lambda e_{traces n} + x_{n}$
%			\STATE $w_{n}(a) \gets w_{n}(a) + \alpha \delta e_{traces n}$
%			\STATE $s \gets s'$
%		\ENDFOR
%%		\STATE Until $s$ is terminal
%
%	\end{algorithmic}
%\end{algorithm}


